The End of a Black Hole's Evaporation -- Part II

We derive an explicit expression for the transition amplitude from black to white hole horizon at the end of Hawking evaporation using covariant loop quantum gravity.

==> The End of a Black Hole's Evaporation - Part II/config.tex <==

\pdfoutput=1

% for quotation marks (english style)
\usepackage[autostyle, english = british]{csquotes}
\MakeOuterQuote{"}

\usepackage[english]{babel}

\usepackage{graphicx}
\usepackage{adjustbox}
\usepackage{subfigure}
\usepackage{capt-of}
\usepackage{bbm}
\usepackage{amsmath,amssymb,amsfonts,tensor}
\usepackage{xcolor}

% for enumeration styles
\usepackage{enumitem}
\setlist[itemize,1]{topsep=2mm,parsep=-1mm,leftmargin=1.5cm}

\usepackage{physics} % for \bracket \matrixel \Re \Im
\usepackage[percent]{overpic} %writing over pictures
\usepackage{pdfpages}

\usepackage{hyperref}
\usepackage{cleveref}
%\usepackage[applemac]{inputenc}

\hypersetup{colorlinks,citecolor=blue,linkcolor=blue,urlcolor=blue,pdfencoding=auto, psdextra}


\setlength{\paperheight}{11in}  %to avoid hyperref warning

%definitions
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand*{\diff}{\mathop{}\!\mathrm{d}}

\newcommand{\pierre}[1]{\textsf{\color{blue}#1}}
\newcommand{\carlo}[1]{\textsf{\color{olive}#1}}
\newcommand{\farshid}[1]{\textsf{\color{purple}#1}}
\newcommand{\D}{{{\cal D}_\gamma^{(j)}}}
\newcommand{\Df}{{\cal D}_\gamma^{(j_{\mathrm{f}})}}
\newcommand{\DF}{{\cal D}_\gamma^{(j_{\mathrm{F}})}}


